A Unified Architecture of Semantic Segmentation and Hierarchical Generative Adversarial Networks for Expression Manipulation

Editing facial expressions by only changing what we want is a long-standing research problem in Generative Adversarial Networks (GANs) for image manipulation. Most of the existing methods that rely only on a global generator usually suffer from changing unwanted attributes along with the target attributes. Recently, hierarchical networks that consist of both a global network dealing with the whole image and multiple local networks focusing on local parts are showing success. However, these methods extract local regions by bounding boxes centred around the sparse facial key points which are non-differentiable, inaccurate and unrealistic. Hence, the solution becomes sub-optimal, introduces unwanted artefacts degrading the overall quality of the synthetic images. Moreover, a recent study has shown strong correlation between facial attributes and local semantic regions. To exploit this relationship, we designed a unified architecture of semantic segmentation and hierarchical GANs. A unique advantage of our framework is that on forward pass the semantic segmentation network conditions the generative model, and on backward pass gradients from hierarchical GANs are propagated to the semantic segmentation network, which makes our framework an end-to-end differentiable architecture. This allows both architectures to benefit from each other. To demonstrate its advantages, we evaluate our method on two challenging facial expression translation benchmarks, AffectNet and RaFD, and a semantic segmentation benchmark, CelebAMask-HQ across two popular architectures, BiSeNet and UNet. Our extensive quantitative and qualitative evaluations on both face semantic segmentation and face expression manipulation tasks validate the effectiveness of our work over existing state-of-the-art methods.

==> figs/proposed_method_rumi.tex <==
\section{Proposed Method}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/proposed_pipeline.pdf}
    \caption{Pipeline showing the proposed method.}
    \label{fig:proposed_pipeline}
\end{figure*}

Figure \ref{fig:proposed_pipeline} shows an overview of the proposed method. As seen in the figure, our hierarchical model consists of one global and four local GANs, a fusion network and a semantic segmentation network. Given a target expression label $\y_t$ and an input image $\x_s$, the objective is to synthesise an image, $\x_t$, which bears the target label, is of high-quality and preserves the identity of $\x_s$. xn this facial expression manipulation scenario, our method is trained on unpaired images. Our hierarchical framework enables it to learn global features as well as local details.
....

\subsection{Global Network} 
The global network serves the purpose of extracting global features of the image. Existing methods mostly consist only of this single network that operates on the whole image. Among these, we chose the StarGAN \cite{choi2018stargan} architecture as our global network. This network consist of a generator, $\G_{global}$, and a discriminator, $\D_{global}$. $\G_{global}$ takes the original image, $\x_s$, as input and generates an image with the target expression label $\y_t$. The translated image, $\x_{global}$, is then passed to $\D_{global}$, which is trained to distinguish between real and fake images and contains an auxiliary expression classifier. $\x_{global}$ is then fused with the output of the local networks to be synthesise the final image, $\x_t$. 
....

\subsection{Local Branch}
Recent studies mostly consist only of a single global network as described above However, these methods tend to generate artifacts and blurs especially around local areas, such as eyes, nose and mouth, where most of the manipulation takes place. These local regions contain essential information that are related to both expression and identity . Hence, we propose a hierarchical architecture, which takes into account these features with the addition of local networks that operate on crucial regions. Our local brach is formed by these local networks and a semantic segmentation that extracts the regions of interest.
...

\noindent\textbf{Semantic Segmentation Network.}
Recent studies that propose architectures with local focuses \cite{yi2019apdrawinggan, wu2020efgan}, extract the local regions in fixed-sized rectangular forms where the centres are defined by landmark locations. However, this approach is sub-optimal as it can lead to artifacts as seen in Figure \ref{fig:motivation} and may not contain the region of interest due to the predefined size. 
xn this respect, to obtain the local regions, we perform semantic segmentation on the input images. We employ the BiSeNet \cite{yu2018bisenet} architecture trained on the CelebAMask-HQ dataset \cite{lee2020celebamask} to extract these local facial regions. 
The left and right eye regions consist of pixels labeled as the corresponding eye and eyebrow, while the mouth area contains the inner mouth and lips pixels. The extracted four local regions, $\x_{left\_eye}, \x_{right\_eye}, \x_{nose}, \x_{mouth}$, are cropped to the contents and resized to the size of $64\times64$.


\noindent\textbf{Local Networks.} Alongside the global network, the proposed architecture contains four local networks that operate on different facial regions extracted by the semantic segmentation network. 
Each of the four networks consists of a generator $\G_{local}=\{\G_{left\_eye}, \G_{right\_eye}, \G_{nose}, \G_{mouth}\}$ and a discriminator $\D_{local}=\{\D_{left\_eye}, \D_{right\_eye}, \D_{nose}, \D_{mouth}\}$. 
As in the global network, we employed the StarGAN \cite{choi2018stargan} architecture for our local networks. Each component of $\G_{local}$ takes as input the corresponding local region and translates it according to the given target label $\y_t$. These generated local regions are stitched together with regard to their original locations. 
The fixed-size rectangular regions extracted by the approach followed by APDrawingGAN \cite{yi2019apdrawinggan} and EF-GAN\cite{wu2020efgan} yield overlapping regions. This can lead to artifacts and blurry results on the overlaps. However, in our case, this problem is mitigated since the regions are extracted semantically and hence do not intersect with each other.  
%\textcolor{blue}{We need to explain how the stitching is done. xs there any issue with the existing method while stitching the network?}
The resulting image, $\x_{local}$, is then concatenated with $\x_{global}$ to be passed to the fusion network.
....



\subsection{Fusion Network}
We use a fusion network in order to fuse together the images generated by $\G_{local}$ and $\G_{global}$, respectively. This fusion network takes as input the concatenation of $\x_{local}$ and $\x_{global}$ and consists of two convolution blocks and four residual blocks followed by a convolution layer.
This network generates the final image $\x_t$, which is passed to the discriminator $\D_{final}$, 
....

\subsection{Loss Functions}

The loss functions to train the proposed method contains three main terms, which are further explained below. 
Our method forms a hierarchical architecture, which consist of a set of discriminators $\D:\{\D_{global}, \D_{local}, \D_{final}\}$ and generators, $\G:\{\G_{global}, \G_{local}, \G_{fusion}\}$, where $\G_{local}:\{\G_{left\_eye}, \G_{right\_eye}, \G_{nose}, \G_{mouth}\}$. The method takes as input  the target label, $\y_t$, and the real image, $\x_s$, which is partitioned by the semantic segmentation network into $\x_{local}:\{\x_{left\_eye}, \x_{right\_eye}, \x_{nose}, \x_{mouth}\}$.

\noindent\textbf{Adversarial Loss.} The adversarial loss trains the discriminator to distinguish between real and fake images. ...

\begin{equation}
\begin{split}
    \mathcal{L}_{adv}=&\mathbb{E}_{\x_s} [\log(D({\x_s}))] \\ 
    &+ \mathbb{E}_{\x_s,\y_t} [\log(1 - \D(\G_{rgb}(\x_s, \y_t))]
\label{eqn:adv_loss}
\end{split}
\end{equation}

\noindent\textbf{Classification Loss.} Besides being realistic, in expression translation the synthesised image, $\x_t$, should bear the given target expression, $\y_t$. Hence, we add an auxiliary classifier, $\D^{cls}$, on top of $\D$, which guides $\G$ to generate images that will be confidently classified as $\y_t$. This classification loss is defined as follows:

\begin{equation}
    \mathcal{L}_{cls}= \mathbb{E}_{\x_s, \y_t} [\log(\D^{cls}(\y_t|\G(\x_s, \y_t)))]
\label{eqn:cls_loss}
\end{equation}


\noindent\textbf{Reconstruction Loss.} xn order to preserve the identity while translating the facial expression, we employ the cycle loss \cite{zhu2017cyclegan}. This loss is defined as

\begin{equation}
    \mathcal{L}_{rec}=\mathbb{E}_{\x_s}[\|\x_s-\hat{\x_s}\|_1] 
\label{eqn:res_loss}
\end{equation}

where $\hat{\x_s}$ is obtained by $\G(\x_t, \y_s)$. Here $\x_t$ is the generated image and $\y_s$ is the  expression of the input image, $\x_s$. 

\noindent\textbf{Overall Training Objective.} The overall objective loss is summarised as

\begin{equation}
    {\mathcal{L} = \lambda_{adv}}{\mathcal{L}_{adv}} + {\lambda_{cls}}{\mathcal{L}_{cls}} + {\lambda_{rec}}{\mathcal{L}_{rec}}
\label{eqn:obj_loss}
\end{equation}

